Interactive GDPR-Compliant Privacy Policy Generation for Software Applications

Software applications are designed to assist users in conducting a wide range of tasks or interactions. They have become prevalent and play an integral part in people's lives in this digital era. To use those software applications, users are sometimes requested to provide their personal information. As privacy has become a significant concern and many data protection regulations exist worldwide, software applications must provide users with a privacy policy detailing how their personal information is collected and processed. We propose an approach that generates a comprehensive and compliant privacy policy with respect to the General Data Protection Regulation (GDPR) for diverse software applications. To support this, we first built a library of privacy clauses based on existing privacy policy analysis. We then developed an interactive rule-based system that prompts software developers with a series of questions and uses their answers to generate a customised privacy policy for a given software application. We evaluated privacy policies generated by our approach in terms of readability, completeness and coverage and compared them to privacy policies generated by three existing privacy policy generators and a Generative AI-based tool. Our evaluation results show that the privacy policy generated by our approach is the most complete and comprehensive.

==> sections/criteria3-results.tex <==
\begin{table*}[ht]
    \centering
    \caption{Some examples of quoted statements from the privacy policies.}
    \label{tab:criteria3-examples}
    \resizebox{6in}{!}{%
        \footnotesize
        \begin{tabular}{@{}ll@{}}
        \toprule
        \multicolumn{1}{c}{\textbf{Privacy policy generator}} & \multicolumn{1}{c}{\textbf{Quoted statement}}    \\ \midrule
        Moodle (original) \cite{Moodle}                                    & \begin{tabular}[c]{@{}l@{}}Moodle Pty Ltd and its affiliated companies (“Moodle”, “we” or “us”), is the company at the heart of the open source \\ Moodle Project: empowering educators to improve our world. This privacy notice sets out how Moodle collects and \\ uses information about you when you use our products and services (“services”) and why we collect certain personal data. \end{tabular} \\ \midrule
        PPGen (our approach)                                 & \begin{tabular}[c]{@{}l@{}}This privacy policy explains how Moodle Pty Ltd (“Moodle Pty Ltd”, “we” or “us”) collects and uses information \\ about you when you use our products and services (“services”) and why we collect certain personal data.\end{tabular} \\ \midrule
        PrivacyPolicies \cite{PrivacyPolicies2022}                                       & \begin{tabular}[c]{@{}l@{}}''Company (referred to as either "the Company", "We", "Us" or "Our" in this Agreement) refers to Moodle Pty Ltd, \\ Moodle Pty Ltd PO Box 303 West Perth WA 6872 Australia.\end{tabular} \\ \midrule
        Termly \cite{Termly2022}                                               & \begin{tabular}[c]{@{}l@{}}This privacy notice for Moodle Pty Ltd ("Company," "we," "us," or "our"), describes how and why we might collect,\\ store, use, and/or share ("process") your information when you use our services ("Services"), ...\end{tabular} \\ \midrule
        TermsFeed \cite{TermsFeed2023}                                            & \begin{tabular}[c]{@{}l@{}}Company (referred to as either "the Company", "We", "Us" or "Our" in this Agreement) refers to Moodle Pty Ltd, \\ Moodle Pty Ltd PO Box 303 West Perth WA 6872 Australia.\end{tabular} \\ \bottomrule
    \end{tabular}%
}
\end{table*}

\begin{comment}
\begin{table*}[!htbp]
	\centering
	\caption{The evaluation results on coverage.}
	\label{tab:criteria3-results}
	\begin{tabular}{@{}lccccc@{}}
		\toprule
		\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Metric}}}                                                                             & \multicolumn{5}{c}{\textbf{Privacy policy generators}}                                                                                                                                                            \\ \cmidrule(l){2-6} 
		\multicolumn{1}{c}{}                                                                                                             & \textbf{\begin{tabular}[c]{@{}c@{}}Moodle\\ (original)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RQA-PPGen\\ (our study)\end{tabular}} & \textbf{PrivacyPolicies} & \textbf{Termly} & \textbf{TermsFeed} \\ \midrule
		\textbf{General   information}                                                                                                   & \textbf{}                                                            & \textbf{}                                                                & \textbf{}                & \textbf{}       & \textbf{}          \\
		\textgreater Effective/Last updated date provided                                                                                & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater General information of the controller                                                                               & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Personal data provision agreement                                                                                   & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\ \midrule
		\textbf{Personal data collection}                                                                                                &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater Definition of personal data                                                                                         & Y                                                                    & Y                                                                        & Y                        & N               & Y                  \\
		\textgreater Purposes of collection                                                                                              & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Special categories of personal data                                                                                 & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Type of personal data collected                                                                                     & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Collecting personal data from individuals                                                                           & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\begin{tabular}[c]{@{}l@{}}\textgreater Collecting personal data by partners/\\ third parties/data collection tools\end{tabular} & N                                                                   & W                                                                        & Y                        & Y               & Y                  \\
		\begin{tabular}[c]{@{}l@{}}\textgreater Collecting personal data by email \\ communication/direct marketing\end{tabular}         & N                                                                   & W                                                                        & N                       & N              & N                 \\ \midrule
		\textbf{Personal data use}                                                                                                       &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater Purposes of use                                                                                                     & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Share with third parties                                                                                            & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Share with service providers                                                                                        & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\begin{tabular}[c]{@{}l@{}}\textgreater Share with third parties outside \\ the scope of this privacy policy\end{tabular}        & N                                                                   & N                                                                        & N                       & N              & N                 \\ \midrule
		\textbf{Personal data storage}                                                                                                   &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater Purposes of storage                                                                                                 & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Personal data storage methods                                                                                       & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Purposes of retention                                                                                               & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Personal data retention methods                                                                                     & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\ \midrule
		\textbf{Personal data transfer}                                                                                                  &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater Transfer outside Europe                                                                                             & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\ \midrule
		\textbf{Individual rights}                                                                                                       &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater General information of individual rights                                                                            & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Right to access                                                                                                     & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Right to judicial review                                                                                            & Y                                                                    & Y                                                                        & N                        & N               & N                  \\
		\textgreater Right to rectification                                                                                              & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Right to delete/erasure/right to be forgotten                                                                       & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Right to restrict of processing                                                                                     & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Right to object to processing                                                                                       & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Right to object to automated processing                                                                             & Y                                                                    & Y                                                                        & N                        & N               & N                  \\
		\textgreater Right to data portability                                                                                           & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Withdraw consent                                                                                                    & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\
		\textgreater Request related to individual rights                                                                                & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\ \midrule
		\textbf{Children's data}                                                                                                         & \multicolumn{1}{l}{}                                                 & \multicolumn{1}{l}{}                                                     & \multicolumn{1}{l}{}     &                 &                    \\
		\textgreater Do not collect children's data                                                                                      & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\ \midrule
		\textbf{Complaint handling}                                                                                                      &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater With the controller                                                                                                 & Y                                                                    & Y                                                                        & N                        & N               & N                  \\
		\textgreater With a supervisory authority                                                                                        & Y                                                                    & Y                                                                        & N                        & N               & N                  \\
		\textgreater Verification before processing requests                                                                             & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\ \midrule
		\textbf{Personal data protection}                                                                                                &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater Security measures                                                                                                   & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Notification of data breaches                                                                                       & N                                                                    & N                                                                        & N                        & N               & N                  \\ \midrule
	\end{tabular}
\end{table*}

\begin{table*}[!htbp]
	\centering
	\begin{tabular}{@{}p{5.7cm}ccccc@{}}
		\toprule
		\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Metric}}}                                                                             & \multicolumn{5}{c}{\textbf{Privacy policy generators}}                                                                                                                                                            \\ \cmidrule(l){2-6} 
		\multicolumn{1}{c}{}                                                                                                             & \textbf{\begin{tabular}[c]{@{}c@{}}Moodle\\ (original)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}RQA-PPGen\\ (our study)\end{tabular}} & \textbf{PrivacyPolicies} & \textbf{Termly} & \textbf{TermsFeed} \\ \midrule
		\textbf{Contact information}                                                                                                     &                                                                      &                                                                          &                          &                 &                    \\
		\textgreater Controller                                                                                                          & Y                                                                    & Y                                                                        & Y                        & Y               & Y                  \\
		\textgreater Controller representative                                                                                           & N                                                                    & W                                                                        & N                        & N               & N                  \\
		\textgreater DPO                                                                                                                 & Y                                                                    & Y                                                                        & N                        & Y               & N                  \\ \bottomrule
	\end{tabular} 

\end{table*}
\end{comment}

